Mining Path Association Rules in Large Property Graphs (with Appendix)

How can we mine frequent path regularities from a graph with edge labels and vertex attributes? The task of association rule mining successfully discovers regular patterns in item sets and substructures. Still, to our best knowledge, this concept has not yet been extended to path patterns in large property graphs. In this paper, we introduce the problem of path association rule mining (PARM). Applied to any \emph{reachability path} between two vertices within a large graph, PARM discovers regular ways in which path patterns, identified by vertex attributes and edge labels, co-occur with each other. We develop an efficient and scalable algorithm PIONEER that exploits an anti-monotonicity property to effectively prune the search space. Further, we devise approximation techniques and employ parallelization to achieve scalable path association rule mining. Our experimental study using real-world graph data verifies the significance of path association rules and the efficiency of our solutions.

==> algorithms/frequentattribute.tex <==
 \begin{algorithm}[!t] 
	\caption{Frequent attribute discovery}	\label{alg:frequentattribute}
		\DontPrintSemicolon
			    %\SetKwInOut{Input}{input}
	            %\SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	            %\Input{Graph $\graph$, min support $\minsup$}
              
              ${\mathcal C} \gets \forall a \in \attributes$\\
              ${\pathpatterns}_0 \gets \varnothing$\\
              \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  ${\pathpatterns}_0 \gets {\pathpatterns}_0 \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup$)}\\
                  ${\mathcal C} \gets$ {\sf GenerateCandidate($\attributes_S$)}\\
              }
               \For{$\elabel \in \elabels$}{
                    $(\edges_F,\attributes_T)  \gets$ {\sf MatchedEdges($\elabel$)}\\
               }
              %{\bf end procedure}
\end{algorithm}


==> algorithms/kleenepathdiscovery.tex <==
\begin{algorithm}[!t] 
	\caption{Frequent Kleene path pattern discovery}	\label{alg:kleenepathpattern}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	          %  \Input{Graph $\graph$, min support $\minsup$, length $\minlen$}
              ${\pathpatterns}^* \gets \varnothing$\\
                 $\vertices_T \gets${\sf BFS($\elabels_F, \graph, \minlen$)}\\
              
              ${\mathcal C} \gets \forall p$ compuated by $\elabels_F, \attributes_T, \pathpatterns_0$\\
              \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  ${\pathpatterns}^* \gets {\pathpatterns}^* \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup, \vertices_T$)}\\
                  ${\mathcal C} \gets$ {\sf HorizontalExtend(${\pathpatterns}^*$)}\\
                }
            %   \For{$c, c' \in \mathcal C$}{
            %   $i \gets 0$\\
            %       \For{$\elabel \in \mathcal N$}{
                  
            %         \For{$v \in V$}{
            %             \If{$A(v) \subseteq c$ and $A(v')$}{
            %                 $i \gets i+1$\\
            %             }
            %           }
                     
            %           \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
            %   }
                    
            %   \While{1}{
            %   ${\mathcal C} \gets$ {\sf GenerateCandidate($F$)}\\
            %   \If{$\mathcal C = \varnothing$}{\bf{break}}
              
            %   \For{$v \in V$}{
            %      \If{$v.F \subseteq c$ for all $\mathcal C$}{
            %         $i \gets i+1$\\
            %     }
            %     \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %   }
            % }
              
            %{\bf end procedure}
\end{algorithm}


==> algorithms/rulediscovery.tex <==
\begin{algorithm}[!t] 
	\caption{Rule discovery}	\label{alg:rulediscovery}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	          %  \Input{Graph $\graph$, min support $\minsup$, length $\minlen$}
	           % \Output{set of rules}
              %{\bf return} rule;\\
              $\rules \gets \varnothing$\\
               ${\mathcal C} \gets \forall (p \Rightarrow p')$ such that $p,p'$ are unit path patterns $\in \pathpatterns_1 \cup \pathpatterns^*$\\
                \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  $\rules \gets \rules \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup$)}\\
                  ${\mathcal C} \gets \forall (p \Rightarrow p')$ so that either $p$ or $p'$ are horizontally and vertically extended path patterns in $\rules$.\\
              }
               
               
            %       \For{$c, c' \in \mathcal C$}{
            %       $i \gets 0$\\
            %       \For{$\elabel \in \mathcal N$}{
                  
            %         \For{$v \in V$}{
            %             \If{$A(v) \subseteq c$ and $A(v')$}{
            %                 $i \gets i+1$\\
            %             }
            %           }
                     
            %           \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
            %   }
            %   \While{1}{
            %       ${\mathcal C} \gets$ {\sf ExtendCandidate($F$)}\\
            %       \If{$\mathcal C = \varnothing$}{\bf{break}}                 
                  
            %       \For{$v \in V$}{
            %          \If{$v.F \subseteq c$ for all $\mathcal C$}{
            %             $i \gets i+1$\\
            %         }
            %         \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
            %   }
              
              {\sf ComputeMetrics}$(\rules)$\\
              %{\bf end procedure}
\end{algorithm}


==> algorithms/simplepathdiscovery.tex <==
\begin{algorithm}[!t] 
	\caption{Frequent simple path pattern discovery}	\label{alg:simplepathpattern}
		\DontPrintSemicolon
			    \SetKwInOut{Input}{input}
	            \SetKwInOut{Output}{output}
	             \SetKwFunction{Expand}{Expand}
	            %\Input{Graph $\graph$, min support $\minsup$, length $\minlen$}
              
              \For{$i = 1$ to $k$}{
                   $\pathpatterns_{i} \gets \varnothing$\\
                  ${\mathcal C} \gets ${\sf VerticalExtend(${\pathpatterns}_{i-1}$)\\       
                  \While{${\mathcal C} \neq \varnothing$}{
            %   \For{$c \in \mathcal C$}{
            %   $i \gets 0$\\
            %   \For{$v \in V$}{
            %         \If{$A(v) \subseteq c$}{
            %             $i \gets i+1$\\
            %         }
            %       }
            %       \If{$i > \minsup$}{
            %          $F \gets F \cup c$
            %       }
            %       }
                  ${\pathpatterns}_i \gets {\pathpatterns}_i \cup$ {\sf Discovery(${\mathcal C}, \graph, \minsup$)}\\
                  ${\mathcal C} \gets$ {\sf HorizontalExtend(${\pathpatterns}_i$)}\\
                }
                }   
                }
        
                                 
            %       \While{1}{
            %       ${\mathcal C} \gets$ {\sf GenerateCandidate($F$)}\\
            %       \If{$\mathcal C = \varnothing$}{\bf{break}}
                  
            %       \For{$v \in V$}{
            %          \If{$v.F \subseteq c$ for all $\mathcal C$}{
            %             $i \gets i+1$\\
            %         }
            %         \If{$i > \minsup$}{
            %              $F \gets F \cup c$
            %           }
            %       }
                  
            %     }
            %   }
             % {\bf end procedure}
\end{algorithm}


==> tables/approximation_factors_camera_ready.tex <==
\begin{table}[!t]
\vspace{-2mm}
\caption{Impact of approximation factors on accuracy.}\label{table:accuracy_factor}
\vspace{-2mm}
\begin{subtable}[h]{1.0\linewidth}
\scalebox{1}{
\begin{tabular}{l|ll|ll|ll}
\hline
\multirow{2}{*}{$\psi$ and $\rho$}& \multicolumn{2}{|c|}{CR}& \multicolumn{2}{|c|}{SA} & \multicolumn{2}{|c}{CR+SA}\\ 
             & Recall     & Precis & Recall& Precis     & Recall & Precis\\ \hline
0.2	&0.046	&1.0	&0.9999	&0.495	&0.046	&0.500\\
0.4	&0.233	&1.0	&0.9999	&0.999	&0.233	&0.998\\
0.6	&0.532	&1.0	&0.9999	&0.9999	&0.532	&0.9999\\
0.8	&0.797	&1.0	&0.9999	&0.9999	&0.797	&0.9999\\
\hline
\end{tabular}
}
\caption{Nell}\label{table:accuracy_factor_nell}
\end{subtable}
\begin{subtable}[h]{1.0\linewidth}
\scalebox{1}{
\begin{tabular}{l|ll|ll|ll}
\hline
\multirow{2}{*}{$\psi$ and $\rho$} & \multicolumn{2}{|c|}{CR}& \multicolumn{2}{|c|}{SA} & \multicolumn{2}{|c}{CR+SA}\\ 
    & Recall     & Precis & Recall& Precis     & Recall & Precis\\ \hline
0.2	&1.0	&1.0	&1.0	&0.978	&1.0	&0.978\\
0.4	&1.0	&1.0	&1.0	&0.882	&1.0	&0.882\\
0.6	&1.0	&1.0	&1.0	&0.938	&1.0	&0.938\\
0.8	&1.0	&1.0	&0.978	&1.0	&0.978	&1.0\\
\hline
\end{tabular}
}
\caption{MiCo}\label{table:accuracy_factor_mico}
\end{subtable}
% \begin{subtable}[h]{1.0\linewidth}
% \scalebox{1}{
% \begin{tabular}{l|ll|ll|ll}
% \hline
% \multirow{2}{*}{$\psi$ and $\rho$} & \multicolumn{2}{|c|}{CR}& \multicolumn{2}{|c|}{SA} & \multicolumn{2}{|c}{CR+SA}\\ 
%              & Recall     & Precis & Recall& Precis     & Recall & Precis\\ \hline
% 0.2	&1.0	&1.0		&1.0	&1.0	&1.0	&1.0\\
% 0.4	&1.0	&1.0		&1.0	&1.0	&1.0	&1.0\\
% 0.6	&1.0	&1.0		&1.0	&1.0	&1.0	&1.0\\
% 0.8	&1.0	&1.0		&1.0	&1.0	&1.0	&1.0\\
% \hline
% \end{tabular}
% }
% \caption{DBpedia}\label{table:accuracy_factor_dbpedia}
% \end{subtable}
% \begin{subtable}[h]{1.0\linewidth}
% \scalebox{1}{
% \begin{tabular}{l|ll|ll|ll}
% \hline
% \multirow{2}{*}{$\psi$ and $\rho$} & \multicolumn{2}{|c|}{CR}& \multicolumn{2}{|c|}{SA} & \multicolumn{2}{|c}{CR+SA}\\ 
%              & Recall     & Precis & Recall& Precis     & Recall & Precis\\ \hline
% 0.2	&1.0	&1.0	&0.934	&0.983	&0.934	&0.983\\
% 0.4	&1.0	&1.0	&0.967	&0.983	&0.967	&0.983\\
% 0.6	&1.0	&1.0	&0.984	&0.986	&0.984	&0.984\\
% 0.8	&1.0	&1.0	&0.984	&0.984	&0.984	&0.984\\
% \hline
% \end{tabular}
% }
% \caption{Pokec}\label{table:accuracy_factor_pokec}
%\end{subtable}
\vspace{-8mm}
\end{table}

==> tables/memory_synthetic.tex <==
\begin{table}[!t]
\vspace{-2mm}
\caption{Memory usage on synthetic graphs [GB]}\label{table:memoryusage}
\vspace{-4mm}
\begin{tabular}{l|rrrr}
\hline
& \multicolumn{1}{c}{Nell} & \multicolumn{1}{c}{MiCo}& \multicolumn{1}{c}{DBpedia} & \multicolumn{1}{c}{Pokec} \\ \hline
Ours & 11.1 & 0.57& 23.9 & 6.4\\
Ours w/ CR & 4.2& 0.55 &21.5& 6.4 \\
Ours w/ SA &5.6& 0.56 & 23.8 &  6.1\\
Ours w/ CR+SA &2.4& 0.53 &21.5 & 6.1 \\
\hline
\end{tabular}
\vspace{-2mm}
\end{table}

==> tables/runtime_csm.tex <==
\begin{table}[!h]
\vspace{-2mm}
\caption{Run time comparison with CSM-A [sec].}\label{table:comparisoncsm}
%All algorithms run on a single thread.
\vspace{-2mm}
\begin{tabular}{l|rrrr}
\hline
& \multicolumn{1}{c}{Nell} & \multicolumn{1}{c}{MiCo}& \multicolumn{1}{c}{DBpedia} & \multicolumn{1}{c}{Pokec} \\ \hline
CSM-A & 835.9 & 228.1 & 1,593 & 848,899\\
Ours w/ CR+SA &419.3& 234.7 & 48,079 & 13,365 \\
\hline
\end{tabular}
\vspace{-2mm}
\end{table}
